M$^2$-ViT: Accelerating Hybrid Vision Transformers with Two-Level Mixed Quantization

Although Vision Transformers (ViTs) have achieved significant success, their intensive computations and substantial memory overheads challenge their deployment on edge devices. To address this, efficient ViTs have emerged, typically featuring Convolution-Transformer hybrid architectures to enhance both accuracy and hardware efficiency. While prior work has explored quantization for efficient ViTs to marry the best of efficient hybrid ViT architectures and quantization, it focuses on uniform quantization and overlooks the potential advantages of mixed quantization. Meanwhile, although several works have studied mixed quantization for standard ViTs, they are not directly applicable to hybrid ViTs due to their distinct algorithmic and hardware characteristics. To bridge this gap, we present M$^2$-ViT to accelerate Convolution-Transformer hybrid efficient ViTs with two-level mixed quantization. Specifically, we introduce a hardware-friendly two-level mixed quantization (M$^2$Q) strategy, characterized by both mixed quantization precision and mixed quantization schemes (i.e., uniform and power-of-two), to exploit the architectural properties of efficient ViTs. We further build a dedicated accelerator with heterogeneous computing engines to transform our algorithmic benefits into real hardware improvements. Experimental results validate our effectiveness, showcasing an average of $80\%$ energy-delay product (EDP) saving with comparable quantization accuracy compared to the prior work.

==> section/Abstract.tex <==
\begin{abstract}
 % Vision Transformers (ViTs) have achieved great success in the computer vision field. However, their intensive computation and huge storage requirements have become the bottlenecks of deploying ViTs on resource-constrained edge devices. To alleviate these limitations, various light and efficient ViTs have emerged as promising alternatives. The state-of-the-art (SOTA) one, EfficientViT achieves improved accuracy with hardware-friendly and quantization-friendly operations, which makes quantization possible. Nonetheless, existing quantization schemes for EfficientViT are uniform and cannot fully exploit the potential opportunity for mixed quantization. Thus, at the algorithm level, we propose a hardware-friendly double-mixed quantization scheme (DMQS) based on the properties of EfficientViT. Besides, at the hardware level, we design a dedicated accelerator based on the proposed DMQS to facilitate EfficientViT’s efficient deployment. Extensive experimental results consistently demonstrate the effectiveness of our DMQS and accelerator. Particularly, compared with the SOTA quantization design for EfficientViT, Trio-ViT, we achieve an average$\downarrow45\%$ EDP drop, with only an average $\downarrow0.18\%$ accuracy drop.

Vision Transformers (ViTs) have achieved great success in the computer vision field. However, their intensive computations and huge memory costs challenge their deployment on edge devices. To address this, efficient ViTs have emerged, which typically incorporate Convolution-Transformer hybrid architectures to enhance both accuracy and hardware efficiency. Concurrently, model quantization, which converts floating-point weights and activations to integers, offers an alternative way to facilitate ViTs' deployment.
To marry the hardware efficiency of both efficient ViT architectures and quantization, Trio-ViT has been developed to investigate quantization and acceleration opportunities dedicated to efficient ViTs. Despite its effectiveness, Trio-ViT mainly focuses on uniform quantization while overlooking the potential advantages of mixed quantization. To bridge this gap, we present M$^2$-ViT, an acceleration framework for Convolution-Transformer hybrid efficient ViTs with double-mixed quantization.
Specifically, we introduce a hardware-friendly double-mixed quantization (M$^2$Q) strategy, which exploits the architectural properties of efficient ViTs to implement quantization with both mixed \textit{bit widths} and mixed \textit{schemes}. Furthermore, we build a reconfigurable accelerator with heterogeneous computing engines, aiming to transform our algorithmic benefits into real hardware improvements.
Experimental results highlight the effectiveness of our M$^2$-ViT framework, showcasing an average $45\%$ energy-delay product (EDP) saving with comparable quantization accuracy when compared with Trio-ViT.

\end{abstract}

==> tables/alg_computation_cost.tex <==
\begin{table}[!t]
\centering
\setlength{\tabcolsep}{4pt}
\caption{Computational cost of EFFICIENTVIT with different quantization schemes} \vspace{-0.8em}
\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cccc}
\Xhline{3\arrayrulewidth}
\multicolumn{2}{c|}{\textbf{Operation numbers (10$^8$)}} & \textbf{8bit$\times$8bit} & \textbf{4bit$\times$8bit}  & \textbf{Shift}    & \textbf{\begin{tabular}[c]{@{}c@{}}Overall computational\\ cost ($\mu$J)\end{tabular} }     \\ \hline \hline
 B1-r224     & \begin{tabular}[c]{@{}c@{}}TrioViT\cite{triovit}\\ Ours\end{tabular}       & \begin{tabular}[c]{@{}c@{}}4.954\\ 2.345\end{tabular}  & \begin{tabular}[c]{@{}c@{}}-\\ 0.263\end{tabular} & \begin{tabular}[c]{@{}c@{}}-\\ 2.345\end{tabular} & \begin{tabular}[c]{@{}c@{}}67.824\\ \textbf{54.473}\end{tabular} \\ \hline

 B1-r256      &\begin{tabular}[c]{@{}c@{}}TrioViT\cite{triovit}\\ Ours\end{tabular}       & \begin{tabular}[c]{@{}c@{}}6.47\\ 3.063\end{tabular}  & \begin{tabular}[c]{@{}c@{}}-\\ 0.344\end{tabular} & \begin{tabular}[c]{@{}c@{}}-\\ 3.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}88.586\\ \textbf{71.148}\end{tabular}\\ \hline

B1-r288      &\begin{tabular}[c]{@{}c@{}}TrioViT\cite{triovit}\\ Ours\end{tabular}       & \begin{tabular}[c]{@{}c@{}}8.189\\ 3.877\end{tabular}  & \begin{tabular}[c]{@{}c@{}}-\\ 0.435\end{tabular} & \begin{tabular}[c]{@{}c@{}}-\\ 3.877\end{tabular} & \begin{tabular}[c]{@{}c@{}}112.116\\ \textbf{90.047}\end{tabular}\\ \hline

B2-r224      &\begin{tabular}[c]{@{}c@{}}Trio-ViT\cite{triovit}\\ Ours\end{tabular}       & \begin{tabular}[c]{@{}c@{}}15.32\\ 7.38\end{tabular}  & \begin{tabular}[c]{@{}c@{}}-\\ 0.56\end{tabular} & \begin{tabular}[c]{@{}c@{}}-\\ 7.38\end{tabular} & \begin{tabular}[c]{@{}c@{}}209.756\\ \textbf{169.41}\end{tabular}\\
 \hline
\multicolumn{2}{c|}{\textbf{Unit Cost ($10^{-4}$ nJ/op)}}            & 1.4977     & 0.749     & 0.869          & -           \\

\Xhline{3\arrayrulewidth}
\end{tabular}} \label{tab:alg_com_cost} \vspace{-1.7em}
\end{table}

==> tables/hw_breakdown.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1.5pt}
\caption{Area and Power Breakdown of our M$^2$ViT accelerator} \vspace{-0.8em}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\Xhline{3\arrayrulewidth}
\textbf{M$^2$ViT}                                                            & \textbf{Component}   & \textbf{Area (mm$^2$)}                                                       & \textbf{Power (mW)}    \\ \hline \hline 
\textbf{Control} & \begin{tabular}[c]{@{}c@{}}Controller  \\ Computating Core Controller\end{tabular} & 0.001 &0.274

                        \\ \hline
\textbf{ Buffers}  & \begin{tabular}[c]{@{}c@{}}Input Buffer\\Weight Buffer (Uniform)\\ Weight Buffer (APoT) \\ Auxiliary Buffer\end{tabular} & \begin{tabular}[c]{@{}c@{}}3.340\end{tabular} & \begin{tabular}[c]{@{}c@{}}1643.6\end{tabular}  \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Computing \\  Engines\end{tabular}} & \begin{tabular}[c]{@{}c@{}} Multiplication Array (MPMA)\\ Shifter and Adder Tree (SAT)  \end{tabular}  &  \begin{tabular}[c]{@{}c@{}} 0.202\\ 0.129  \end{tabular}   &  \begin{tabular}[c]{@{}c@{}} 79.282\\ 44.038  \end{tabular} \\ \hline
\textbf{Total} & \multicolumn{3}{c}{TSMC 28nm: Area = 3.672  mm$^2$, Power = 1.767 W }      \\ 

 \Xhline{3\arrayrulewidth}                                                             
\end{tabular}} \label{tab:hw_breakdown} \vspace{-1.5em}
\end{table}
